Laplacian Matrix for Dimensionality Reduction and Clustering

Many problems in machine learning can be expressed by means of a graph with nodes representing training samples and edges representing the relationship between samples in terms of similarity, temporal proximity, or label information. Graphs can in turn be represented by matrices. A special example is the Laplacian matrix, which allows us to assign each node a value that varies only little between strongly connected nodes and more between distant nodes. Such an assignment can be used to extract a useful feature representation, find a good embedding of data in a low dimensional space, or perform clustering on the original samples. In these lecture notes we first introduce the Laplacian matrix and then present a small number of algorithms designed around it.

==> Figures/InANutshell-LEM.Tags.tex <==
\def\TagBib{}% bibtex key
\def\TagRef{Wiskott, 2017, unpubl.}% human readable reference
\def\TagURL{}% url
\def\TagDat{2017-12-05}% date in format YYYY-MM-DD
\def\TagFig{}% figure or table number, e.g. 'Fig.~2'
\def\TagCLI{\CLWFree}%
\def\TagCLIURL{\CLWFreeURL}%
\def\TagCLIColor{\CLWFreeColor}% copyright and license infos, typically a macro such as \CLWFree


==> Figures/InANutshell-SC.Tags.tex <==
\def\TagBib{}% bibtex key
\def\TagRef{Wiskott, 2017, unpubl.}% human readable reference
\def\TagURL{}% url
\def\TagDat{2017-12-06}% date in format YYYY-MM-DD
\def\TagFig{}% figure or table number, e.g. 'Fig.~2'
\def\TagCLI{\CLWFree}%
\def\TagCLIURL{\CLWFreeURL}%
\def\TagCLIColor{\CLWFreeColor}% copyright and license infos, typically a macro such as \CLWFree


==> Figures/SimpleDirectedGraph3Nodes.Tags.tex <==
\def\TagBib{}% bibtex key
\def\TagRef{Wiskott, 2017, unpubl.}% human readable reference
\def\TagURL{}% url
\def\TagDat{2017-11-27}% date in format YYYY-MM-DD
\def\TagFig{}% figure or table number, e.g. 'Fig.~2'
\def\TagCLI{\CLWFree}%
\def\TagCLIURL{\CLWFreeURL}%
\def\TagCLIColor{\CLWFreeColor}% copyright and license infos, typically a macro such as \CLWFree


==> Figures/SimpleUndirectedGraph3Nodes.Tags.tex <==
\def\TagBib{}% bibtex key
\def\TagRef{Wiskott, 2017, unpubl.}% human readable reference
\def\TagURL{}% url
\def\TagDat{2017-11-27}% date in format YYYY-MM-DD
\def\TagFig{}% figure or table number, e.g. 'Fig.~2'
\def\TagCLI{\CLWFree}%
\def\TagCLIURL{\CLWFreeURL}%
\def\TagCLIColor{\CLWFreeColor}% copyright and license infos, typically a macro such as \CLWFree


==> Images/BelkinNiyogi-2002-NIPS-LEM-Fig01.Tags.tex <==
% The .Tags.tex files should be formatted as follows
\def\TagBib{BelkinNiyogi-2002}% bibtex key
\def\TagRef{Belkin \& Niyogi, 2002, NIPS}% human readable reference, e.g. 'Wiskott, 2017', where year indicates first publication (may not contain \emph, include \hspace{0em} to allow linebreaks in long urls)
\def\TagURL{http://papers.nips.cc/paper/1961-laplacian-eigenmaps-and-spectral-techniques-for-embedding-and-clustering.pdf}% url, replace '~' by '\%7e', '_' should work (is there a '_' in \TagRef?) see http://tex.stackexchange.com/questions/10858/url-with-tilde-character or rather https://tools.ietf.org/html/rfc3986#page-12
\def\TagURLText{http://papers.nips.cc/paper/1961-\allowbreak{}laplacian-\allowbreak{}eigenmaps-\allowbreak{}and-\allowbreak{}spectral-\allowbreak{}techniques-\allowbreak{}for-\allowbreak{}embedding-\allowbreak{}and-\allowbreak{}clustering.pdf}% 
\def\TagDat{2017-11-13}% date of download or figure creation in format YYYY-MM-DD
\def\TagFig{\EG{Fig.}{Abb.}~1}% figure or table number, e.g. '\EG{Fig.}{Abb.}~2'
\def\TagCLI{\CUnclear}%
\def\TagCLIURL{\CUnclearURL}%
\def\TagCLIColor{\CUnclearColor}% copyright and license infos, typically a macro such as \CCBY


==> Images/BelkinNiyogi-2003-NeurComp-LEM.Tags.tex <==
% The .Tags.tex files should be formatted as follows
\def\TagBib{BelkinNiyogi-2003}% bibtex key
\def\TagRef{Belkin \& Niyogi, 2003, Neur.\ Comp.}% human readable reference, e.g. 'Wiskott, 2017', where year indicates first publication (may not contain \emph, include \hspace{0em} to allow linebreaks in long urls)
\def\TagURL{https://pdfs.semanticscholar.org/989a/f45f8242b96cecb91d48b85620e7322e4aa7.pdf}% url, replace '~' by '\%7e', '_' should work (is there a '_' in \TagRef?) see http://tex.stackexchange.com/questions/10858/url-with-tilde-character or rather https://tools.ietf.org/html/rfc3986#page-12
\def\TagDat{2017-11-13}% date of download or figure creation in format YYYY-MM-DD
\def\TagFig{}% figure or table number, e.g. '\EG{Fig.}{Abb.}~2'
\def\TagCLI{\CUnclear}%
\def\TagCLIURL{\CUnclearURL}%
\def\TagCLIColor{\CUnclearColor}% copyright and license infos, typically a macro such as \CCBY


==> Images/HeNiyogi-2004-NIPS-LPP.Tags.tex <==
% The .Tags.tex files should be formatted as follows
\def\TagBib{HeNiyogi-2004}% bibtex key
\def\TagRef{He and Niyogi, 2004, NIPS}% human readable reference, e.g. 'Wiskott, 2017', where year indicates first publication (may not contain \emph, include \hspace{0em} to allow linebreaks in long urls)
\def\TagURL{http://papers.nips.cc/paper/2359-locality-preserving-projections.pdf}% url, replace '~' by '\%7e', '_' should work (is there a '_' in \TagRef?) see http://tex.stackexchange.com/questions/10858/url-with-tilde-character or rather https://tools.ietf.org/html/rfc3986#page-12
\def\TagDat{2017-11-20}% date of download or figure creation in format YYYY-MM-DD
\def\TagFig{}% figure or table number, e.g. '\EG{Fig.}{Abb.}~2'
\def\TagCLI{\CUnclear}%
\def\TagCLIURL{\CUnclearURL}%
\def\TagCLIColor{\CUnclearColor}% copyright and license infos, typically a macro such as \CCBY


==> Images/Iris_dataset_scatterplot.Tags.tex <==
% The .Tags.tex files should be formatted as follows
\def\TagBib{}% bibtex key
\def\TagRef{Nicoguaro, 2016, Wikimedia}% human readable reference, e.g. 'Wiskott, 2017', where year indicates first publication (may not contain \emph, include \hspace{0em} to allow linebreaks in long urls)
\def\TagURL{https://commons.wikimedia.org/wiki/File:Iris_dataset_scatterplot.svg}% url, replace '~' by '\%7e', '_' should work (is there a '_' in \TagRef?) see http://tex.stackexchange.com/questions/10858/url-with-tilde-character or rather https://tools.ietf.org/html/rfc3986#page-12
\def\TagDat{2017-12-02}% date of download or figure creation in format YYYY-MM-DD
\def\TagFig{}% figure or table number, e.g. '\EG{Fig.}{Abb.}~2'
\def\TagCLI{\CCBYFour}%
\def\TagCLIURL{\CCBYFourURL}%
\def\TagCLIColor{\CCBYFourColor}% copyright and license infos, typically a macro such as \CCBY


==> Images/Specclus_iriscluster.Tags.tex <==
% The .Tags.tex files should be formatted as follows
\def\TagBib{}% bibtex key
\def\TagRef{Sigbert, 2014, Wikimedia}% human readable reference, e.g. 'Wiskott, 2017', where year indicates first publication (may not contain \emph, include \hspace{0em} to allow linebreaks in long urls)
\def\TagURL{https://commons.wikimedia.org/wiki/File:Specclus_iriscluster.svg}% url, replace '~' by '\%7e', '_' should work (is there a '_' in \TagRef?) see http://tex.stackexchange.com/questions/10858/url-with-tilde-character or rather https://tools.ietf.org/html/rfc3986#page-12
\def\TagDat{2017-12-02}% date of download or figure creation in format YYYY-MM-DD
\def\TagFig{}% figure or table number, e.g. '\EG{Fig.}{Abb.}~2'
\def\TagCLI{\CCBYSAFour}%
\def\TagCLIURL{\CCBYSAFourURL}%
\def\TagCLIColor{\CCBYSAFourColor}% copyright and license infos, typically a macro such as \CCBY


==> TEX-macros/myBasics.tex <==
% packages Merlin Schüler has used for reinforcement learning exercises
\usepackage{tikz}
\usetikzlibrary{automata, positioning}
\usepackage{tabu}
\usepackage{pgfplots}

% to permit many counters and avoid the errror message "! No room for a new \count"
\usepackage{etex}

\input{./TEX-macros/myColors}
\input{./TEX-macros/myFigureStyle}
%\input{myHyperref}

\usepackage{endnotes}

% to set pararagraph transitions
\setlength{\parindent}{0em}
\setlength{\parskip}{1ex plus 1.5ex minus0.5ex}

% to process utf8 files
\input{./TEX-macros/myUTF8}

% the root directory
\input{./TEX-macros/myRootDir}

% the ignore macro
\providecommand{\ignore}[1]{}

% the name of the HU in English
\providecommand{\HUE}{Humboldt-University Berlin}
%\providecommand{\HUE}{Humboldt-Universit{\"a}t zu Berlin}

% the name of the INI in German and English
\providecommand{\INIG}{Institut f\"ur Neuroinformatik}
\providecommand{\INIE}{Institute for Neural Computation}

% the name of the RUB in German and English
\providecommand{\RUBG}{Ruhr-Universit\"at Bochum}
\providecommand{\RUBE}{Ruhr University Bochum}

% a math point or comma
\providecommand{\myPoint}{\EG{.}{,\!}}
\providecommand{\myComma}{\EG{,\!}{.}}

% correct spacing after a reference to be included with (\input{ref.tex})
%\newcommand{\CorrectRefSpacing}{\hspace{-0.8ex}}
\providecommand{\CorrectRefSpacing}{}

% Copyright infos
\usepackage{ifthen}
\provideboolean{ShowCLInfos}
\setboolean{ShowCLInfos}{false}

% \CPL stands for Copyright Protection Level and is a variable indicating the degree to
% which copyright protection takes effect.  (0) No protection.  That is used for student
% versions of lecture notes and slides.  (1) Mark copyrighted material, i.e. show the
% protected images but mark somehow that they are protected.  This is used for my
% personal versions of lecture notes and slides.  (2) Protect, i.e. disclose copyright
% protected material.  This is used for publicly available versions of lecture notes and
% slides.

% \RefCLInfo stands for Reference Copyright and License Info.  This should generally be
% given under all figures, above the figure caption.

% \RefCLInfoCite includes a cite command and should only be used in a context where
% bibtex can be used.  This is mainly at the end of \notes{} part of slides.

% There are four versions of it.

% (A) For scientific material of other people.  That should be cited in any case.  Always
% shown and set in black.

% (B) For illustrative images from other than scientifically relevant sources,
% e.g. images on section title slides.  Always shown and set in gray.

% (C) For my own published material, where others may have copyright but I may use it.
% That should generally be cited but may be omitted on slides, if there is a general
% source reference in the lower right.  Set in black.

% (D) For my own unpublished material.  That might not be cited.  Set in gray.

\providecommand{\RefSizeA}{\RefSize}
\providecommand{\RefSizeC}{\RefSizeB}
\providecommand{\RefSizeD}{\RefSizeB}
\providecommand{\ResetTags}{%
% The .Tags.tex files should be formatted as follows
\def\TagBib{}% Bibtex key
\def\TagRef{}% human readable Reference, e.g. 'Wiskott, 2017', where year indicates first publication (may not contain \emph, include \hspace{0em} to allow linebreaks in long urls)
\def\TagURL{}% URL, replace '~' by '\%7e', '_' should work (is there a '_' in \TagRef?) see http://tex.stackexchange.com/questions/10858/url-with-tilde-character or rather https://tools.ietf.org/html/rfc3986#page-12
\def\TagURLText{}% Text version of URL with \allowbreak{} in it at positions to break the URL without adding a hyphen '-', if URL cannot be broken properly.
\def\TagDat{}% Date of download in format YYYY-MM-DD, but only for web pages etc, journal papers don't need that
\def\TagFig{}% Figure or table number, e.g. '\EG{Fig.}{Abb.}~2'
\def\TagCLI{\CUnclear}% Copyright and License Infos, typically a macro such as \CCBY, see ~/TEX/macros/myBasics.tex
\def\TagCLIURL{\CUnclearURL}%
\def\TagCLIColor{\CUnclearColor}%
}
\ResetTags

\def\AddEndnote{%
\ifthenelse{\NOT\equal{\TagURL}{}}{% {A: If a URL is given define \TagURLNote.
\edef\TagURLNote{%
\TagFigString% Add \TagFigString in any case
\noexpand\ifthenelse{\noexpand\equal{\TagCLIColor}{}}{}{% {B}{B: If \TagCLIColor is given, add copyright notice.
, \noexpand\textcolor{\TagCLIColor}{\noexpand\copyright}%
\noexpand\ifthenelse{\noexpand\equal{\TagCLI}{}}{}{% {C}{C: If \TagCLI is given, add copyright text.
\noexpand\ifthenelse{\noexpand\equal{\TagCLIURL}{}}{% {D: If \TagCLIURL is given, add link to copyright text.
\ \TagCLI%
}{% :D}{D:
\ \noexpand\href{\TagCLIURL}{\TagCLI}%
}% :D}
}% :C}
}% :B}
, \noexpand\ifthenelse{\noexpand\equal{\TagURLText}{}}{\noexpand\url{\TagURL}}{\noexpand\href{\TagURL}{\noexpand\texttt{\TagURLText}}}% Add URL in any case.
}%
\expandafter\expandafter\expandafter\endnote\expandafter\expandafter\expandafter{\expandafter\TagRef\TagURLNote}%
% See http://stackoverflow.com/questions/4016725/latex-immediate-evaluation for an explanation of the \expandafter usage.
}{}% :A}{A}
}

%\providecommand{\RefCLInfoText}[3][]{%
%\IfFileExists{#3.Tags}{%
%\ResetTags%
%\input{#3.Tags}%
%%\ifthenelse{\equal{\TagRef}{}}{\def\TagRef{\url{\TagURL}\ifthenelse{\equal{\TagDat}{}}{}{, \TagDat}}}{}%
%\ifthenelse{\equal{#1}{}}{}{\def\TagFig{#1}}%
%\ifthenelse{\equal{\TagFig}{}}{\edef\TagFigString{}}{\edef\TagFigString{, \TagFig}}%
%\ifthenelse{\equal{\TagRef}{}}{\edef\TagRef{\texttt{\TagURL} \TagDat}}{}%
%% Das Folgende funktioniert nicht, vermutlich muss da irgendwo ein \noexpand hin oder so.
%%\ifthenelse{\equal{\TagRef}{}}{
%%  \edef\TagRef{\TagURL
%%    \ifthenelse{\equal{\TagDat}{}}{}{, \TagDat}
%%}}{}%
%\vspace{-0.2ex}%
%\centerline{%
%\href{\TagURL}{%
%(\TagRef%
%\TagFigString%
%%\ifthenelse{\equal{\CPL}{1}}{%
%\ifthenelse{\equal{\TagCLI}{}}{}{, \copyright\ \href{\TagCLIURL}{\TagCLI}}%
%%}{}%\ifthenelse{\equal{\CPL}{1}}{%
%)%
%}% \href{\TagURL}{%
%\AddEndnote%
%}%\centerline{\RefSizeX%
%}{}%\IfFileExists{#3.Tags}{%
%}
\providecommand{\RefCLInfoA}[3][]{\textcolor{black}{{\RefSizeA\RefCLInfoText[#1]{#2}{#3}}}}
\providecommand{\RefCLInfoB}[3][]{\textcolor{lightgray}{{\RefSizeB\RefCLInfoText[#1]{#2}{#3}}}}
\providecommand{\RefCLInfoC}[3][]{%
\ifthenelse{\equal{\CPL}{1}}{%
\textcolor{lightgray}{{\RefSizeC\RefCLInfoText[#1]{#2}{#3}}}%
}{}% \ifthenelse{\equal{\CPL}{1}}{%
}
\providecommand{\RefCLInfoD}[3][]{%
\ifthenelse{\equal{\CPL}{1}}{%
\textcolor{lightgray}{{\RefSizeC\RefCLInfoText[#1]{#2}{#3}}}%
}{}% \ifthenelse{\equal{\CPL}{1}}{%
}

% Die \RefCLInfoCiteX-Befehle nicht in eine \caption Umgebung schreiben, sondern unter
% die Abbildung, weil sonst die endnotes immer zweimal auftauchen.
% Beispiel: \centerline{\RefSize\RefCLInfoCiteA[Fig.~1]{}{./Images/SebekBortelEtAl-2018}}
\providecommand{\RefCLInfoCore}[3][]{%
\ifthenelse{\equal{#1}{}}{}{\def\TagFig{#1}}% initialize \TagFig with optional argument if given
\ifthenelse{\equal{\TagFig}{}}{\edef\TagFigString{}}{\edef\TagFigString{, \TagFig}}% add comma in front of \TagFig(String) if not empty
\ifthenelse{\equal{\TagRef}{}}{\edef\TagRef{\texttt{\TagURL} \TagDat}}{}% if \TagRef is empty, create it from \TagURL and \TagDat
\hspace{0ex}% is for some strange reason necessary to get the indentation right if not preceeded by text
%
% print preceeding 'Figure: ' or something similar
\ifthenelse{\equal{#2}{}}{}{% if second argument is not empty ...
#2: % ... print second argument, e.g. 'Figure', without URL to original document
%\ifthenelse{\equal{\TagURL}{}}{#2}{\href{\TagURL}{#2}}: % ... print second argument, e.g. 'Figure', possibly with URL to original document
}% \ifthenelse{\equal{#2}{}}{}{%
%
% print reference
\ifthenelse{\equal{\TagBib}{}}{%
\ifthenelse{\equal{\TagRef}{}}{(unknown}{(\TagRef}% print \TagRef if available and no \TagBib is available
}{% \ifthenelse{\equal{\TagBib}{}}{%
(\citeauthor{\TagBib}, \citeyear{\TagBib}% 
}% \ifthenelse{\equal{\TagBib}{}}{%
%
% print optional parameter, e.g. 'Fig. 1'
\TagFigString%
% print copyright info
\ifthenelse{\equal{\TagCLI}{}}{}{, \textcolor{\TagCLIColor}{\copyright} \href{\TagCLIURL}{\TagCLI}}%
%
% add clickable URL
\ifthenelse{\equal{\TagURL}{}}{}{, \href{\TagURL}{URL}}%
)%
\AddEndnote%
}

\providecommand{\RefCLInfoText}[3][]{%
\IfFileExists{#3.Tags}{%
\ResetTags%
\input{#3.Tags}% read tags file
\def\TagBib{}%
\RefCLInfoCore[#1]{#2}{#3}%
}{}%\IfFileExists{#3.Tags}{%
}

\providecommand{\RefCLInfoCite}[3][]{%
\IfFileExists{#3.Tags}{%
\ResetTags%
\input{#3.Tags}% read tags file
\RefCLInfoCore[#1]{#2}{#3}%
}{}%\IfFileExists{#3.Tags}{%
}

\providecommand{\RefCLInfoCiteA}[3][]{\RefCLInfoCite[#1]{#2}{#3}}
\providecommand{\RefCLInfoCiteB}[3][]{\textcolor{lightgray}{\RefCLInfoCiteA[#1]{#2}{#3}}}
\providecommand{\RefCLInfoCiteC}[3][]{\RefCLInfoCiteA[#1]{#2}{#3}}
%\providecommand{\RefCLInfoCiteD}[3][]{\textcolor{lightgray}{\RefCLInfoCiteC[#1]{#2}{#3}}}
\providecommand{\RefCLInfoCiteD}[3][]{%
\IfFileExists{#3.Tags}{%
\ResetTags%
\input{#3.Tags}%
%\ifthenelse{\equal{#1}{}}{}{\def\TagFig{#1}}%
%\ifthenelse{\equal{\TagFig}{}}{\edef\TagFigString{}}{\edef\TagFigString{, \TagFig}}%
%\ifthenelse{\equal{\TagRef}{}}{\edef\TagRef{\texttt{\TagURL} \TagDat}}{}%
%\hspace{0ex}% is for some strange reason necessary to get the indentation right if not preceeded by text
%\ifthenelse{\NOT\equal{\TagURL}{}}{%
%\href{\TagURL}{#2}%
%}{#2}:% \ifthenelse{\NOT\equal{\TagURL}{}}{%
%\ifthenelse{\NOT\equal{\TagBib}{}}{%
%\cite[][\TagFig]{\TagBib}%
%}{% \ifthenelse{\NOT\equal{\TagBib}{}}{%
%\ifthenelse{\NOT\equal{\TagRef}{}}{%
%(\TagRef)%
%}{% \ifthenelse{\NOT\equal{\TagRef}{}}{%
%\ (unknown)%
%}% \ifthenelse{\NOT\equal{\TagRef}{}}{%
%}% \ifthenelse{\NOT\equal{\TagBib}{}}{%
%\AddEndnote%
\ifthenelse{\equal{\TagCLI}{}}{}{ \textcolor{\TagCLIColor}{\copyright} \href{\TagCLIURL}{\TagCLI}}%
%\ifthenelse{\equal{\TagCLI}{}\OR\equal{\TagURL}{}}{}{, }%
%\ifthenelse{\equal{\TagURL}{}}{}{ available at \url{\TagURL}}%
%.%
}{}%\IfFileExists{#3.Tags}{%
}


%\providecommand{\CLInfo}[1]{\ifthenelse{\boolean{ShowCLInfos}}{\vspace{-0.5ex}\centerline{\textcolor{lightgray}{\RefSizeB(#1)}}}{}} % obsolete
%\providecommand{\CInfo}[1]{\CLInfo{#1}} % obsolete
%\providecommand{\CNotice}[1]{\CLInfo{#1}} % obsolete
%\providecommand{\SourceFigure}[1]{\CLInfo{#1}} % obsolete
%\providecommand{\SourceImage}[1]{\CLInfo{#1}} % obsolete

% Copyright icons
% CC0
\providecommand{\CCNull}{CC0}
\providecommand{\CCNullURL}{https://creativecommons.org/share-your-work/public-domain/cc0/}
\providecommand{\CCNullColor}{green}
% public domain
\providecommand{\CPublicDomain}{public domain}
\providecommand{\CPublicDomainURL}{https://creativecommons.org/share-your-work/public-domain/pdm/}
\providecommand{\CPublicDomainColor}{green}
% CC BY 2.0
\providecommand{\CCBYTwo}{CC BY 2.0}
\providecommand{\CCBYTwoURL}{https://creativecommons.org/licenses/by/2.0/}
\providecommand{\CCBYTwoColor}{green}
% CC BY 4.0
\providecommand{\CCBYFour}{CC BY 4.0}
\providecommand{\CCBYFourURL}{https://creativecommons.org/licenses/by/4.0/}
\providecommand{\CCBYFourColor}{green}
% CC BY
\providecommand{\CCBY}{CC BY 4.0}
\providecommand{\CCBYURL}{https://creativecommons.org/licenses/by/4.0/}
\providecommand{\CCBYColor}{green}
% CC BY-SA 2.5
\providecommand{\CCBYSATwoFive}{CC BY-SA 2.5}
\providecommand{\CCBYSATwoFiveURL}{https://creativecommons.org/licenses/by-sa/2.5/}
\providecommand{\CCBYSATwoFiveColor}{green}
% CC BY-SA 3.0
\providecommand{\CCBYSAThree}{CC BY-SA 3.0}
\providecommand{\CCBYSAThreeURL}{https://creativecommons.org/licenses/by-sa/3.0/}
\providecommand{\CCBYSAThreeColor}{green}
% CC BY-SA 4.0
\providecommand{\CCBYSAFour}{CC BY-SA 4.0}
\providecommand{\CCBYSAFourURL}{https://creativecommons.org/licenses/by-sa/4.0/}
\providecommand{\CCBYSAFourColor}{green}
% CC BY-SA
\providecommand{\CCBYSA}{CC BY-SA 4.0}
\providecommand{\CCBYSAURL}{https://creativecommons.org/licenses/by-sa/4.0/}
\providecommand{\CCBYSAColor}{green}
% LW free (for figures I have created)
\providecommand{\CLWFree}{\CCBYSA}
\providecommand{\CLWFreeURL}{\CCBYSAURL}
\providecommand{\CLWFreeColor}{\CCBYSAColor}
% CC BY-NC-SA 3.0
\providecommand{\CCBYNCSAThree}{CC BY-NC-SA 3.0}
\providecommand{\CCBYNCSAThreeURL}{https://creativecommons.org/licenses/by-nc-sa/3.0/}
\providecommand{\CCBYNCSAThreeColor}{green}
% unclear
\providecommand{\CUnclear}{} % unclear
\providecommand{\CUnclearURL}{}
\providecommand{\CUnclearColor}{} % red
% non-free
\providecommand{\CNonFree}{} % non-free
\providecommand{\CNonFreeURL}{}
\providecommand{\CNonFreeColor}{} % red


==> TEX-macros/myBeamerStyle.tex <==
\input{./TEX-macros/myBasics}
\let\footnote=\endnote
%\input{myLatin}
\input{./TEX-macros/myUTF8}
\input{./TEX-macros/myMath}
\input{./TEX-macros/myLatexOrPdflatex}
%\input{myThumbpdf}
\input{./TEX-macros/myColors}
\input{./TEX-macros/myGraphicx}
\input{./TEX-macros/myRotating}
\input{./TEX-macros/myUSEnglish}

\usepackage{ifthen}

% dummy \dir definition
\def\dir {/home/wiskott}

% if making handouts
\mode<handout>{
 % resize to a4 
 % this screws up the hyperref placement, but that shouldn't matter for handouts
 \usepackage{pgfpages}
 \pgfpagesuselayout{resize to}[a4paper,border shrink=5mm,landscape]
 % show notes
 %\setbeameroption{show notes}
}

% setting of section title
\newcommand{\SecTitleNote}[1]{Section title: \textbf{#1}}

% figure citation command in notes
\newcommand{\FigCite}[3]{\cite[#1][#3]{#2}}

% poster macros
\newcommand{\Poster}[1]{} % redefine this if you want a poster


% macros to control which slides to include
\newcommand{\InsertFrom}[3]{\ifthenelse{\not\value{#1}<#2}{#3}{}}
\newcommand{\InsertTo}[3]{\ifthenelse{\not\value{#1}>#2}{#3}{}}
\newcommand{\InsertFromTo}[4]{\ifthenelse{\not\value{#1}<#2\and\not\value{#1}>#3}{#4}{}}

\newlength{\freeheight}
\setlength{\freeheight}{0.93\textheight}


%% Title Page

\setbeamercolor{title}{fg=black}
\setbeamerfont{title}{series=\bfseries}
\newcommand{\TitleHeader}[1]{\title{#1 \vspace{-0.5em}}\Source{}}
\newcommand{\Author}[1]{\author{#1 \vspace{-0.5em}}}
\renewcommand{\And}{\and}
\newcommand{\Institute}[1]{\institute{#1}}
\newcommand{\MakeTitle}{\maketitle}
\newcommand{\Thanks}[1]{\vspace{-10ex}\begin{center}\scriptsize #1\end{center}\vspace{10ex}}

% Authors
\newboolean{Appleby-Peter}
\newboolean{Azizi-Amir}
\newboolean{Bandt-Christoph}
\newboolean{Bayati-Mehdi}
\newboolean{Beisswanger-Elena}
\newboolean{Berkes-Pietro}
\newboolean{Blaschke-Tobias}
\newboolean{Brecht-Michael}
\newboolean{Cheng-Sen}
\newboolean{Dahne-Sven}
\newboolean{Escalante-Alberto}
\newboolean{Franzius-Mathias}
\newboolean{Kempermann-Gerd}
\newboolean{Lezius-Susanne}
\newboolean{Melchior-Jan}
\newboolean{Michaelis-Christian}
\newboolean{Neher-Torsten}
\newboolean{Rasch-Malte}
\newboolean{Richthofer-Stefan}
\newboolean{Schoenfeld-Fabian}
\newboolean{Sprekeler-Henning}
\newboolean{Weghenkel-Bjoern}
\newboolean{Wichmann-Felix}
\newboolean{Wilbert-Niko}
\newboolean{Zito-Tiziano}
%\newcommand{\IncludeCoAuthor}[2]{\hspace*{0.2em} #1 \hspace*{0.2em}}
\newcommand{\IncludeCoAuthor}[2]{\hspace*{0.2em}
  \begin{minipage}[t]{0.15\textwidth}
    \centerline{\IfFileExists{/home/wiskott/TEX/macros/PortraitImages/#2}{\includegraphics[height=\textwidth]{/home/wiskott/TEX/macros/PortraitImages/#2}}{\phantom{blank}}}
    \vspace{-1ex}
    \centerline{\scriptsize #1}
    \vspace{1ex}
  \end{minipage}
  \hspace*{0.2em}}
\newcommand{\IncludeCoAuthorB}[2]{\hspace*{0.2em}
  \begin{minipage}[t]{0.15\textwidth}
    \centerline{\IfFileExists{/home/wiskott/TEX/macros/PortraitImages/#2}{\includegraphics[height=\textwidth]{/home/wiskott/TEX/macros/PortraitImages/#2}}{\phantom{blank}}}
    \vspace{-1ex}
    \centerline{\scriptsize #1}
    \vspace{1ex}
  \end{minipage}}
\newcommand{\AuthorList}{Laurenz Wiskott\vspace{2ex}\\  
\ifthenelse{\boolean{Appleby-Peter}}{\IncludeCoAuthor{Peter~Appleby}{}}{}%
\ifthenelse{\boolean{Azizi-Amir}}{\IncludeCoAuthor{Azizi~Amir}{AmirAzizi.png}}{}%
\ifthenelse{\boolean{Bandt-Christoph}}{\IncludeCoAuthor{Christoph~Bandt}{}}{}%
\ifthenelse{\boolean{Bayati-Mehdi}}{\IncludeCoAuthor{Mehdi~Bayati}{MehdiBayati.jpg}}{}%
\ifthenelse{\boolean{Beisswanger-Elena}}{\IncludeCoAuthor{Elena~Bei\ss{}wanger}{}}{}%
\ifthenelse{\boolean{Berkes-Pietro}}{\IncludeCoAuthor{Pietro~Berkes}{PietroBerkes-color.jpg}}{}%
\ifthenelse{\boolean{Blaschke-Tobias}}{\IncludeCoAuthor{Tobias~Blaschke}{}}{}%
\ifthenelse{\boolean{Cheng-Sen}}{\IncludeCoAuthor{Sen~Cheng}{SenCheng.jpg}}{}%
\ifthenelse{\boolean{Dahne-Sven}}{\IncludeCoAuthor{Sven~D\"ahne}{SvenDaehne.jpg}}{}%
\ifthenelse{\boolean{Escalante-Alberto}}{\IncludeCoAuthor{Alberto~Escalante}{AlbertoEscalante.jpg}}{}%
\ifthenelse{\boolean{Franzius-Mathias}}{\IncludeCoAuthor{Mathias~Franzius}{MathiasFranzius.jpg}}{}%
\ifthenelse{\boolean{Kempermann-Gerd}}{\IncludeCoAuthor{Gerd~Kempermann}{}}{}%
\ifthenelse{\boolean{Lezius-Susanne}}{\IncludeCoAuthor{Susanne~Lezius}{}}{}%
\ifthenelse{\boolean{Melchior-Jan}}{\IncludeCoAuthor{Jan~Melchior}{JanMelchior.jpg}}{}%
\ifthenelse{\boolean{Michaelis-Christian}}{\IncludeCoAuthor{Christian~Michaelis}{}}{}%
\ifthenelse{\boolean{Neher-Torsten}}{\IncludeCoAuthor{Torsten~Neher}{TorstenNeher-2011.jpg}}{}%
\ifthenelse{\boolean{Rasch-Malte}}{\IncludeCoAuthor{Malte~Rasch}{}}{}%
\ifthenelse{\boolean{Richthofer-Stefan}}{\IncludeCoAuthor{Stefan~Richthofer}{StefanRichthofer.jpg}}{}%
\ifthenelse{\boolean{Schoenfeld-Fabian}}{\IncludeCoAuthor{Fabian~Sch\"onfeld}{FabianSchoenfeld.jpg}}{}%
\ifthenelse{\boolean{Sprekeler-Henning}}{\IncludeCoAuthor{Henning~Sprekeler}{HenningSprekeler-small.jpg}}{}%
\ifthenelse{\boolean{Weghenkel-Bjoern}}{\IncludeCoAuthor{Björn~Weghenkel}{BjoernWeghenkel.jpg}}{}%
\ifthenelse{\boolean{Wilbert-Niko}}{\IncludeCoAuthor{Niko~Wilbert}{NikoWilbert.jpg}}{}%
\ifthenelse{\boolean{Zito-Tiziano}}{\IncludeCoAuthor{Tiziano~Zito}{TizianoZito.jpg}}{}%
}

% Funding Agencies
\newboolean{AvHumboldStiftung}
\newboolean{Wissenschaftskolleg}
\newboolean{VolkswagenStiftung}
\newboolean{BMBF}
\newboolean{RUB}
\newboolean{SFB874}
\newcommand{\FundingList}{
\ifthenelse{\boolean{AvHumboldStiftung}}{Alexander von Humboldt \EG{Foundation}{Stiftung} - Feodor Lynen \EG{Fellowship}{Stipendium} \\ }{}%
\ifthenelse{\boolean{Wissenschaftskolleg}}{\EG{Institute for Advanced Studies Berlin}{Wissenschaftskolleg zu Berlin} - \EG{Fellowship}{Stipendium} \\ }{}%
\ifthenelse{\boolean{VolkswagenStiftung}}{\EG{Volkswagen Foundation - Junior Research Group}{Volkswagen Stiftung - Nachwuchsgruppe} \\ }{}%
\ifthenelse{\boolean{BMBF}}{BMBF - \EG{\ignore{German Federal Ministry of Education and Research - }Bernstein Center for Computational Neuroscience Berlin}{\ignore{Bundesministerium für Bildung und Forschung -}Bernstein Zentrum für Computational Neuroscience Berlin} \\ }{}%
\ifthenelse{\boolean{RUB}}{Ruhr-University Bochum \\ }{}%
\ifthenelse{\boolean{SFB874}}{Deutsche Forschungsgemeinschaft - Sonderforschungsbereich 874 \\ }{}%
}


% Slides
% frame title template WITHOUT subtitles
\setbeamercolor{frametitle}{fg=black}
\setbeamerfont{frametitle}{series=\bfseries}
\setbeamertemplate{frametitle}{
\begin{centering}
%\vspace{1ex}
\insertframetitle
%\vspace{-2ex}
\vspace{-1ex}
\par
\end{centering}
}

\newcommand{\frames}[1]{\begin{frame}[allowframebreaks] #1 \end{frame}}
%\newcommand{\FrameSecTitle}[1]{\frame{#1}}
%\newcommand{\FrameSecSummary}[1]{\frame{#1}}

% don't use linebreaks (\\) in headers, use \mbox instead
% section header
%\newcommand{\SectionHeader}[2][]{\section<presentation>{#2}\frametitle{\LARGE #2}\label{slide:\dir/#1}\Source{}}
\newcommand{\SectionHeader}[2][]{\section{#2}\frametitle{\LARGE #2}\label{slide:\dir/#1}\Source{}}
% section header with authors
%\newcommand{\SectionHeaderTA}[3][]{\section{#2}\frametitle{{\LARGE #2} \\ \centerline{\mbox{{\normalsize \textmd{#3}}}}}\label{slide:\dir/#1}\Source{}}
\newcommand{\SectionHeaderTA}[3][]{\SectionHeader[#1]{#2}}
%\newcommand{\SlideHeader}[2][]{\subsection<presentation>{#2}\frametitle{\large #2}\label{slide:\dir/#1}\Source{}}
\newcommand{\SlideHeader}[2][]{\subsection{#2}\frametitle{\large\rule[-0.4ex]{0em}{0ex} #2}\label{slide:\dir/#1}\Source{}}
% The rule command is necessary to eliminate height differences between titles with and without 'gyp' or other letter that hang below baseline.
% slide header with subtitle
\newcommand{\SlideHeaderWST}[2]{\subsection<presentation>{#1}\frametitle{{\large #1} \\ {\normalsize #2}}\Source{}}

% no indentation of first lines in paragraph
\setlength{\parindent}{0ex}
\setlength\parskip{1ex plus 1.5ex minus 0.5ex}

% no indentation of lists
\setlength{\leftmargini}{0pt} % text is shifted to the left margin
\setlength{\leftmargini}{2.5ex} % bullet point is shifted to the left margin

% summary and reference macros
\newcommand{\iconWidth}{0.15\textwidth}
%\newcommand{\iconWidth}{0.3\textwidth}
\newcommand{\iconHeight}{0.7\textwidth}
\newcommand{\textWidth}{0.8\textwidth}
%\newcommand{\textWidth}{0.65\textwidth}
\newcommand{\SummaryItem}[2]{
\fbox{%
\begin{minipage}[c]{\iconWidth}
\centerline{
 {\includegraphics[keepaspectratio,width=\textwidth,totalheight=\iconHeight]{#1}}
}
\end{minipage}}\hfill
\begin{minipage}[c]{\textWidth}
#2
\end{minipage}\\
}
\newcommand{\TalkSummary}{}
\newcommand{\AddSummaryItem}[1]{\expandafter\def\expandafter\TalkSummary\expandafter{\TalkSummary{}#1}}
\newcommand{\ReferenceItem}[2]{
\fbox{%
\begin{minipage}[c]{\iconWidth}
\centerline{
 {\includegraphics[keepaspectratio,width=\textwidth,totalheight=\iconHeight]{#1}}
}
\end{minipage}}\hfill
\begin{minipage}[c]{\textWidth}
#2
\end{minipage}\\
}
\newcommand{\TalkReferences}{}
\newcommand{\AddReferenceItem}[1]{\expandafter\def\expandafter\TalkReferences\expandafter{\TalkReferences{}#1}}

\newcommand{\SourceRef}[1]{\centerline{\RefSize(#1)}}
\newcommand{\SourceSecTitleImage}[1]{\centerline{\textcolor{lightgray}{\RefSizeB(#1)}}}
%\newcommand{\Source}[1]{\setbeamertemplate{footline}[text line]{this is a test}}
\newcommand{\Source}[1]{\vspace*{-2ex}{\tiny \hfill #1}}
%\newcommand{\Source}[1]{}
\newcommand{\SourceCompare}[2]{\vspace*{-2ex}{\tiny \begin{minipage}{\textwidth}\hfill (#1; \\ \hspace*{\fill} \EG{cf.}{vgl.}\ #2)\end{minipage}}}

\newcommand{\vspaceCorrectEquation}{\vspace{-3ex}}
\newcommand{\vspaceCorrectEqnarray}{\vspace{-4ex}}
\newcommand{\RefAnd}{\&}
\newcommand{\RefSize}{\scriptsize}
\newcommand{\RefSizeB}{\tiny}


% empty head- and footline
\useoutertheme{default}
% no navigation symbols
\setbeamertemplate{navigation symbols}{}

%==============================================================================
% talk time management

\newcounter{BPreviousTotalTimeDesired}
\newcounter{BTimeUsedForThisSlide}
\newcounter{BTotalTimeDesired}
\setcounter{BTotalTimeDesired}{0}

\newcommand{\BTimeUsedForThisSlideIs}[1]{
\setcounter{BTimeUsedForThisSlide}{#1}
\setcounter{BPreviousTotalTimeDesired}{\value{BTotalTimeDesired}}
\addtocounter{BTotalTimeDesired}{#1}
}

\newcommand{\PrintFileAndTotalTimeDesired}[1]{
\ifthenelse{\value{BTimeUsedForThisSlide}=0}{
\immediate\write8{==============================================================================}
\immediate\write8{==============================================================================}
\immediate\write8{WARNING: Slide without time information: #1}
\immediate\write8{==============================================================================}
\immediate\write8{==============================================================================}
}{
\immediate\write8{------------------------------------------------------------------------------}
\immediate\write8{Slide: #1}
\immediate\write8{Total Time: \arabic{BPreviousTotalTimeDesired} + \arabic{BTimeUsedForThisSlide} = \arabic{BTotalTimeDesired} seconds.}
\immediate\write8{------------------------------------------------------------------------------}
}
\setcounter{BTimeUsedForThisSlide}{0}
\setcounter{BPreviousTotalTimeDesired}{\value{BTotalTimeDesired}}
}

%==============================================================================
% lecture notes compatibility

\input{./TEX-macros/myFootnoteAddress}

% variable to decide whether to hide copyright protected material
%obsolete \newboolean{ProtectCopyrights}
%obsolete \setboolean{ProtectCopyrights}{false}
\newcounter{CopyrightProtectionLevel}         
\setcounter{CopyrightProtectionLevel}{0} % 0: no protection; 1: mark but show; 2: mark and hide

\newcommand{\inputSlide}[1]{
\input{\dir/#1}
\PrintFileAndTotalTimeDesired{#1}
}

\newcommand{\inputSlideC}[1]{
\ifthenelse{\value{CopyrightProtectionLevel}<1}{\input{\dir/#1}}{}
\ifthenelse{\value{CopyrightProtectionLevel}=1}{\input{/home/wiskott/PR/General/Talks/Slides/ProtectCopyrights}\input{\dir/#1}}{}
\ifthenelse{\value{CopyrightProtectionLevel}>1}{\input{/home/wiskott/PR/General/Talks/Slides/ProtectCopyrights}}{}
\PrintFileAndTotalTimeDesired{#1}
}
\renewcommand{\inputSlideC}[1]{\inputSlide{#1}}

\providecommand{\LNTime}[1]{}
\providecommand{\LNTimes}[2]{}
\providecommand{\RefToSlidesInHeader}{}
\providecommand{\LNExtra}[1]{}
\providecommand{\LNExtraSection}{}
\providecommand{\markText}[1]{#1}
\providecommand{\paragraph}{}
\providecommand{\markEqnLect}{}
\providecommand{\markEqn}{}

%==============================================================================


==> TEX-macros/myColors.tex <==
%\usepackage{color} % does not provide lightgray, for instance
% see https://en.wikibooks.org/wiki/LaTeX/Colors
%\usepackage[usenames,dvipsnames,svgnames,table]{xcolor} % results in an option clash with the beamer class
\usepackage{xcolor}

\definecolor{myGreen}{RGB}{0,160,0}
\definecolor{myDarkGreen}{RGB}{0,120,0}
\definecolor{myRed}{RGB}{230,0,0}
\definecolor{myDarkRed}{RGB}{180,0,0}
\definecolor{myDarkBlue}{RGB}{0,0,180}
\definecolor{myLightGray}{RGB}{210,210,210}


==> TEX-macros/myFigureStyle.tex <==
\renewcommand{\topfraction}{0.8}
\renewcommand{\bottomfraction}{0.8}
\renewcommand{\textfraction}{0.2}


==> TEX-macros/myFootnoteAddress.tex <==
\providecommand{\myFootnoteAddress}{Institut f\"ur Neuroinformatik, Ruhr-Universit\"at
  Bochum, \url{https://www.ini.rub.de/PEOPLE/wiskott/}.}


==> TEX-macros/myGraphicx.tex <==
% If no protection level has been defined up to this point, then this default value is set.
%\providecommand{\CPL}{2} % X: protection level mechanism not in effect; 0: no protection; 1: mark but show; 2: mark and hide (must come before myGraphicx)

\usepackage{ifthen}

\providecommand{\LNEdition}{Students}
\ifthenelse{\equal{\LNEdition}{Me}}{%
  \providecommand{\CPL}{1} % 0: no protection; 1: mark but show; 2: mark and hide (must come before myGraphicx)
}{%
  \ifthenelse{\equal{\LNEdition}{Students}}{%
    \providecommand{\CPL}{0} % 0: no protection; 1: mark but show; 2: mark and hide (must come before myGraphicx)
  }{%
    \ifthenelse{\equal{\LNEdition}{Public}}{%
      \providecommand{\CPL}{2} % 0: no protection; 1: mark but show; 2: mark and hide (must come before myGraphicx)
    }{%
      \LWUnknownCommandToStopLatexHereBecauseOfWrongEdition
    }}}

% with these definitions latex and pdflatex will try to automatically
% generate graphics files that are missing and store them with double
% an extra .tmp.graphics extensions, such as .fig.tmp.eps (latex) or
% .eps.tmp.pdf (pdflatex), which indicate how the files have been generated
% and that these files can be removed

% if you get the error message `system() disabled' with pdflatex
% try `pdflatex -shell-escape <myfile>'

% if you get segmentation faults with latex when including .jpg or .pdf
% convert .jpg to .pdf using 'convert' and .pdf to .eps using 'pdftops' by hand

% 2016-02-10 I had problem for a long time since sh rather than bash was used.  Now I
% have figured that `bash -c '...' does the trick.  I have not converted all lines to
% that new syntax.

% 2018-04-06 Don't use ~/ in \includegraphics{}.  That does not get resolved.  Use
% /home/wiskott/ instead.

% 2018-04-06 If there is an erro message of the form "!Missing number ..." or so when
% compiling lectureNotes with 'latexmk', then the reason is probably that lectureHandout
% has not been compiled.  Use 'make lectureNotes...' instead.

% 2018-04-06 Don't use ~/ in \DeclareGraphicsRule{}{}{}{} either.  That also
% does not get resolved, despite the bash command.  Use /home/wiskott/ instead.

% include graphics
%\usepackage[pdftex]{graphicx,rotating}
\usepackage{graphicx,rotating}

% if latex
% --------
\ifx\undefined\pdfoutput
\DeclareGraphicsExtensions{.eps,.eps.tmp.eps,.eps.gz,.ps,.ps.tmp.ps,.ps.gz,.fig.tmp.eps,.fig,.fig.gz,.gp.tmp.eps,.gp,.gp.gz,.m.tmp.eps,.m.tmp.eps,.m,.m.gz,.pdf.tmp.eps,.pdf,.png.tmp.eps,.png,.jpg.tmp.eps,.jpg,.gif.tmp.eps,.gif,.pdf.gz,.jpg.gz,.gif.gz,.png.gz}

\DeclareGraphicsRule{*}{eps}{*}{}

% eps
\DeclareGraphicsRule{.eps}{eps}{.eps}{}
\DeclareGraphicsRule{.eps.tmp.eps}{eps}{.eps.tmp.eps}{}
\DeclareGraphicsRule{.eps.gz}{eps}{.eps.tmp.eps.bb}{`bash -c 'file=$(basename #1); file=${file/.eps.gz/.eps}; path=$(dirname #1); cd $path; gunzip -c $file.gz > $file.tmp.eps; cat $file.tmp.eps | grep BoundingBox > $file.tmp.eps.bb; cat $file.tmp.eps'}

% ps
\DeclareGraphicsRule{.ps}{eps}{.ps}{}
\DeclareGraphicsRule{.ps.tmp.ps}{eps}{.ps.tmp.ps}{}
\DeclareGraphicsRule{.ps.gz}{eps}{.ps.tmp.ps.bb}{`bash -c 'file=$(basename #1); file=${file/.ps.gz/.ps}; path=$(dirname #1); cd $path; gunzip -c $file.gz > $file.tmp.ps; cat $file.tmp.ps | grep BoundingBox > $file.tmp.ps.bb; cat $file.tmp.ps'}

% fig
\DeclareGraphicsRule{.fig.tmp.eps}{eps}{.fig.tmp.eps}{}
\DeclareGraphicsRule{.fig}{eps}{.fig.tmp.eps.bb}{`bash -c 'file=$(basename #1); path=$(dirname #1); cd $path; if [ ! -f $file.tmp.eps ] || [ $file.tmp.eps -ot $file ]; then fig2dev -L eps $file $file.tmp.eps; cat $file.tmp.eps | grep BoundingBox > $file.tmp.eps.bb; fi; cat $file.tmp.eps'}
\DeclareGraphicsRule{.fig.gz}{eps}{.fig.tmp.eps.bb}{`bash -c 'file=$(basename #1); file=${file/.fig.gz/.fig}; path=$(dirname #1); cd $path; if [ ! -f $file.tmp.eps ] || [ $file.tmp.eps -ot $file.gz ]; then gunzip -c $file.gz | fig2dev -L eps > $file.tmp.eps; cat $file.tmp.eps | grep BoundingBox > $file.tmp.eps.bb; fi; cat $file.tmp.eps'}

% .m (matlab) -> .eps
\DeclareGraphicsRule{.m.tmp.eps}{eps}{.m.tmp.eps}{}
\DeclareGraphicsRule{.m}{eps}{.m.tmp.eps.bb}{`bash -c 'cat #1 > tmp.m; echo print -depsc #1.tmp.eps >> tmp.m; cat tmp.m | matlab -nosplash; rm tmp.m; cat #1.tmp.eps | grep BoundingBox > #1.tmp.eps.bb; cat #1.tmp.eps'}
\DeclareGraphicsRule{.m.gz}{eps}{.m.tmp.eps.bb}{`srcFile=#1; dstFile=${srcFile/.m.gz/.m}; gunzip -c $srcFile > tmp.m; echo print -depsc $dstFile.tmp.eps >> tmp.m; cat tmp.m | matlab -nosplash; rm tmp.m; cat $dstFile.tmp.eps | grep BoundingBox > $dstFile.tmp.eps.bb; cat $dstFile.tmp.eps}

% gp (gnuplot)
% metapost doesn't work with xdvi but it works with dvips-gv
\DeclareGraphicsRule{.gp.mps.tmp}{eps}{.gp.mps.tmp}{}
\DeclareGraphicsRule{.gp}{mps}{.gp.mps.tmp}{`bash -c 'file=$(basename #1); path=$(dirname #1); cd $path; echo set terminal mp color > tmp.gp; cat $file >> tmp.gp; gnuplot tmp.gp > $file.mp; mpost $file.mp; rm $file.mp $file.mpx; rm $file.log; mv $file.0 $file.mps.tmp; cat $file.mps.tmp'}
\DeclareGraphicsRule{.gp.gz}{eps}{.gp.mps.tmp}{`gzFile=`basename #1`; path=$(dirname #1); nFile=${gzFile/.gp.gz/.gp}; cd $path; echo set terminal mp color > tmp.gp; gunzip -c $gzFile >> tmp.gp; gnuplot tmp.gp > $nFile.mp; mpost $nFile.mp; rm $nFile.mp $nFile.mpx; rm $nFile.log; mv $nFile.0 $nFile.mps.tmp; cat $nFile.mps.tmp}

% gp (gnuplot) this version assumes .gp files that only plot but not postscript
\DeclareGraphicsRule{.gp.tmp.eps}{eps}{.gp.tmp.eps}{}
\DeclareGraphicsRule{.gp}{eps}{.gp.tmp.eps.bb}{`bash -c 'file=$(basename #1); path=$(dirname #1); cd $path; if [ ! -f $file.tmp.eps ] || [ $file.tmp.eps -ot $file ]; then echo 'set size 0.6,0.6; set terminal postscript eps enhanced color' > tmp.gp; cat $file >> tmp.gp; gnuplot tmp.gp > $file.tmp.eps; rm tmp.gp; cat $file.tmp.eps | grep BoundingBox > $file.tmp.eps.bb; fi; cat $file.tmp.eps'}
\DeclareGraphicsRule{.gp.gz}{eps}{.gp.tmp.eps.bb}{`bash -c 'file=$(basename #1); file=${file/.gp.gz/.gp}; path=$(dirname #1); cd $path; if [ ! -f $file.tmp.eps ] || [ $file.tmp.eps -ot $file.gz ]; then echo 'set size 0.6,0.6; set terminal postscript eps enhanced color' > tmp.gp; gunzip -c $file.gz >> tmp.gp; gnuplot tmp.gp > $file.tmp.eps; rm tmp.gp; cat $file.tmp.eps | grep BoundingBox > $file.tmp.eps.bb; fi; cat $file.tmp.eps'}

% gp (gnuplot) this version assumes .gp files that plot in postscript
\DeclareGraphicsRule{.gp.tmp.eps}{eps}{.gp.tmp.eps}{}
\DeclareGraphicsRule{.gp}{eps}{.gp.tmp.eps.bb}{`bash -c 'file=$(basename #1); path=$(dirname #1); cd $path; if [ ! -f $file.tmp.eps ] || [ $file.tmp.eps -ot $file ]; then gnuplot $file > $file.tmp.eps; cat $file.tmp.eps | grep BoundingBox > $file.tmp.eps.bb; fi; cat $file.tmp.eps'}
\DeclareGraphicsRule{.gp.gz}{eps}{.gp.tmp.eps.bb}{`bash -c 'file=$(basename #1); file=${file/.gp.gz/.gp}; path=$(dirname #1); cd $path; if [ ! -f $file.tmp.eps ] || [ $file.tmp.eps -ot $file.gz ]; then echo 'set size 0.6,0.6; set terminal postscript eps enhanced color' > tmp.gp; gunzip -c $file.gz >> tmp.gp; gnuplot tmp.gp > $file.tmp.eps; rm tmp.gp; cat $file.tmp.eps | grep BoundingBox > $file.tmp.eps.bb; fi; cat $file.tmp.eps'}

% pdf
\DeclareGraphicsRule{.pdf.tmp.eps}{eps}{.pdf.tmp.eps}{}
\DeclareGraphicsRule{.pdf}{eps}{.pdf.tmp.eps.bb}{`pdftops -eps #1 #1.tmp.eps; cat #1.tmp.eps | grep BoundingBox > #1.tmp.eps.bb; cat #1.tmp.eps}
\DeclareGraphicsRule{.pdf.gz}{eps}{.pdf.tmp.eps.bb}{`srcFile=#1; dstFile=${srcFile/.pdf.gz/.pdf}; gunzip $srcFile; pdftops -eps $dstFile $dstFile.tmp.eps; gzip -9 $dstFile; cat $dstFile.tmp.eps | grep BoundingBox > $dstFile.tmp.eps.bb; cat $dstFile.tmp.eps}

% png
\DeclareGraphicsRule{.png.tmp.eps}{eps}{.png.tmp.eps}{}
\DeclareGraphicsRule{.png}{eps}{.png.tmp.eps.bb}{`convert #1 #1.tmp.eps; cat #1.tmp.eps | grep BoundingBox > #1.tmp.eps.bb; cat #1.tmp.eps}
\DeclareGraphicsRule{.png.gz}{eps}{.png.tmp.eps.bb}{`srcFile=#1; dstFile=${srcFile/.png.gz/.png}; gunzip -c $srcFile | convert - $dstFile.tmp.eps; cat $dstFile.tmp.eps | grep BoundingBox > $dstFile.tmp.eps.bb; cat $dstFile.tmp.eps}

% jpg
\DeclareGraphicsRule{.jpg.tmp.eps}{eps}{.jpg.tmp.eps}{}
\DeclareGraphicsRule{.jpg}{eps}{.jpg.tmp.eps.bb}{`convert #1 #1.tmp.eps; cat #1.tmp.eps | grep BoundingBox > #1.tmp.eps.bb; cat #1.tmp.eps}
\DeclareGraphicsRule{.jpg.gz}{eps}{.jpg.tmp.eps.bb}{`srcFile=#1; dstFile=${srcFile/.jpg.gz/.jpg}; gunzip -c $srcFile | convert - $dstFile.tmp.eps; cat $dstFile.tmp.eps | grep BoundingBox > $dstFile.tmp.eps.bb; cat $dstFile.tmp.eps}

% gif
\DeclareGraphicsRule{.gif.tmp.eps}{eps}{.gif.tmp.eps}{}
\DeclareGraphicsRule{.gif}{eps}{.gif.tmp.eps.bb}{`convert #1 #1.tmp.eps; cat #1.tmp.eps | grep BoundingBox > #1.tmp.eps.bb; cat #1.tmp.eps}
\DeclareGraphicsRule{.gif.gz}{eps}{.gif.tmp.eps.bb}{`srcFile=#1; dstFile=${srcFile/.gif.gz/.gif}; gunzip -c $srcFile | convert - $dstFile.tmp.eps; cat $dstFile.tmp.eps | grep BoundingBox > $dstFile.tmp.eps.bb; cat $dstFile.tmp.eps}

% if pdflatex
% -----------
\else
\usepackage{epstopdf} % permits online generation of graphic files
\epstopdfsetup{suffix=} % avoids using the default extension 'converted-to'
% including pdf files created with xfig causes large files and wrong textures
\DeclareGraphicsExtensions{
  .CFree.pdf,   .CMeFree.pdf,   .CNonFree.pdf,   .pdf,
  .CFree.png,   .CMeFree.png,   .CNonFree.png,   .png,
  .CFree.jpg,   .CMeFree.jpg,   .CNonFree.jpg,   .jpg,
  .CFree.gif,   .CMeFree.gif,   .CNonFree.gif,   .gif,
  .CFree.svg,   .CMeFree.svg,   .CNonFree.svg,   .svg,
  .CFree.fig,   .CMeFree.fig,   .CNonFree.fig,   .fig,
  .CFree.gp,    .CMeFree.gp,    .CNonFree.gp,    .gp,
  .m,
  .CFree.eps,   .CMeFree.eps,   .CNonFree.eps,   .eps,
  .CFree.ps,    .CMeFree.ps,    .CNonFree.ps,    .ps,
  .CFree.pdf.gz,.CMeFree.pdf.gz,.CNonFree.pdf.gz,.pdf.gz,
  .CFree.png.gz,.CMeFree.png.gz,.CNonFree.png.gz,.png.gz,
  .CFree.jpg.gz,.CMeFree.jpg.gz,.CNonFree.jpg.gz,.jpg.gz,
  .CFree.gif.gz,.CMeFree.gif.gz,.CNonFree.gif.gz,.gif.gz,
  .CFree.svg.gz,.CMeFree.svg.gz,.CNonFree.svg.gz,.svg.gz,
  .CFree.fig.gz,.CMeFree.fig.gz,.CNonFree.fig.gz,.fig.gz,
  .CFree.gp.gz, .CMeFree.gp.gz, .CNonFree.gp.gz, .gp.gz,
  .m.gz,
  .CFree.eps.gz,.CMeFree.eps.gz,.CNonFree.eps.gz,.eps.gz,
  .CFree.ps.gz, .CMeFree.ps.gz, .CNonFree.ps.gz, .ps.gz,
}

% make
%\DeclareGraphicsRule{.make} {pdf}{.make.tmp.pdf}{`bash -c 'file=$(basename #1); path=$(dirname #1); cd $path; make -f $file'}

% png
\DeclareGraphicsRule         {.png}   {png}            {.png.\CPL.tmp.png}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.png'}
\DeclareGraphicsRule         {.png.gz}{png}         {.png.gz.\CPL.tmp.png}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.png'}
\DeclareGraphicsRule   {.CFree.png}   {png}      {.CFree.png.\CPL.tmp.png}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.png'}
\DeclareGraphicsRule   {.CFree.png.gz}{png}   {.CFree.png.gz.\CPL.tmp.png}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.png'}
\DeclareGraphicsRule {.CMeFree.png}   {png}    {.CMeFree.png.\CPL.tmp.png}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.png'}
\DeclareGraphicsRule {.CMeFree.png.gz}{png} {.CMeFree.png.gz.\CPL.tmp.png}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.png'}
\DeclareGraphicsRule{.CNonFree.png}   {png}   {.CNonFree.png.\CPL.tmp.png}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.png'}
\DeclareGraphicsRule{.CNonFree.png.gz}{png}{.CNonFree.png.gz.\CPL.tmp.png}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.png'}
%\DeclareGraphicsRule{.png}   {png}{.png}         {}
%\DeclareGraphicsRule{.png.gz}{png}{.png}         {`gunzip #1}

% jpg
\DeclareGraphicsRule         {.jpg}   {jpg}            {.jpg.\CPL.tmp.jpg}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.jpg'}
\DeclareGraphicsRule         {.jpg.gz}{jpg}         {.jpg.gz.\CPL.tmp.jpg}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.jpg'}
\DeclareGraphicsRule   {.CFree.jpg}   {jpg}      {.CFree.jpg.\CPL.tmp.jpg}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.jpg'}
\DeclareGraphicsRule   {.CFree.jpg.gz}{jpg}   {.CFree.jpg.gz.\CPL.tmp.jpg}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.jpg'}
\DeclareGraphicsRule {.CMeFree.jpg}   {jpg}    {.CMeFree.jpg.\CPL.tmp.jpg}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.jpg'}
\DeclareGraphicsRule {.CMeFree.jpg.gz}{jpg} {.CMeFree.jpg.gz.\CPL.tmp.jpg}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.jpg'}
\DeclareGraphicsRule{.CNonFree.jpg}   {jpg}   {.CNonFree.jpg.\CPL.tmp.jpg}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.jpg'}
\DeclareGraphicsRule{.CNonFree.jpg.gz}{jpg}{.CNonFree.jpg.gz.\CPL.tmp.jpg}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.jpg'}
%\DeclareGraphicsRule{.jpg.gz}{jpg}{.jpg}         {`gunzip #1}

% pdf
\DeclareGraphicsRule         {.pdf}   {pdf}            {.pdf.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule         {.pdf.gz}{pdf}         {.pdf.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule   {.CFree.pdf}   {pdf}      {.CFree.pdf.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule   {.CFree.pdf.gz}{pdf}   {.CFree.pdf.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule {.CMeFree.pdf}   {pdf}    {.CMeFree.pdf.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule {.CMeFree.pdf.gz}{pdf} {.CMeFree.pdf.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule{.CNonFree.pdf}   {pdf}   {.CNonFree.pdf.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule{.CNonFree.pdf.gz}{pdf}{.CNonFree.pdf.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
%\DeclareGraphicsRule{.pdf.gz}{pdf}{.pdf}         {`gunzip #1}

% gif
\DeclareGraphicsRule         {.gif}   {png}            {.gif.\CPL.tmp.png}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.png'}
\DeclareGraphicsRule         {.gif.gz}{png}         {.gif.gz.\CPL.tmp.png}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.png'}
\DeclareGraphicsRule   {.CFree.gif}   {png}      {.CFree.gif.\CPL.tmp.png}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.png'}
\DeclareGraphicsRule   {.CFree.gif.gz}{png}   {.CFree.gif.gz.\CPL.tmp.png}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.png'}
\DeclareGraphicsRule {.CMeFree.gif}   {png}    {.CMeFree.gif.\CPL.tmp.png}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.png'}
\DeclareGraphicsRule {.CMeFree.gif.gz}{png} {.CMeFree.gif.gz.\CPL.tmp.png}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.png'}
\DeclareGraphicsRule{.CNonFree.gif}   {png}   {.CNonFree.gif.\CPL.tmp.png}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.png'}
\DeclareGraphicsRule{.CNonFree.gif.gz}{png}{.CNonFree.gif.gz.\CPL.tmp.png}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.png'}
%\DeclareGraphicsRule{.gif}   {png}{.gif.tmp.png}{`bash -c 'file=$(basename #1);                            path=$(dirname #1); cd $path; if [ ! -f $file.tmp.png ] || [ $file.tmp.png -ot $file    ]; then                      convert $file $file.tmp.png; fi'}
%\DeclareGraphicsRule{.gif.gz}{png}{.gif.tmp.png}{`bash -c 'file=$(basename #1); file=${file/.gif.gz/.gif}; path=$(dirname #1); cd $path; if [ ! -f $file.tmp.png ] || [ $file.tmp.png -ot $file.gz ]; then gunzip -c $file.gz | convert -     $file.tmp.png; fi'}

% svg (inkscape)
\DeclareGraphicsRule         {.svg}   {pdf}            {.svg.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule         {.svg.gz}{pdf}         {.svg.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule   {.CFree.svg}   {pdf}      {.CFree.svg.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule   {.CFree.svg.gz}{pdf}   {.CFree.svg.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule {.CMeFree.svg}   {pdf}    {.CMeFree.svg.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule {.CMeFree.svg.gz}{pdf} {.CMeFree.svg.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule{.CNonFree.svg}   {pdf}   {.CNonFree.svg.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule{.CNonFree.svg.gz}{pdf}{.CNonFree.svg.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
%\DeclareGraphicsRule{.svg}   {pdf}{.svg.tmp.pdf}{`bash -c 'file=$(basename #1);                            path=$(dirname #1); cd $path; if [ ! -f $file.tmp.pdf ] || [ $file.tmp.pdf -ot $file    ]; then                                     inkscape --file=$file         --export-area-drawing --export-pdf=$file.tmp.pdf; fi'}
%\DeclareGraphicsRule{.svg.gz}{pdf}{.svg.tmp.pdf}{`bash -c 'file=$(basename #1); file=${file/.svg.gz/.svg}; path=$(dirname #1); cd $path; if [ ! -f $file.tmp.pdf ] || [ $file.tmp.pdf -ot $file.gz ]; then gunzip -c $file.gz > $file.tmp.svg; inkscape --file=$file.tmp.svg --export-area-drawing --export-pdf=$file.tmp.pdf; rm -f $file.tmp.svg; fi'}

% fig
\DeclareGraphicsRule         {.fig}   {pdf}            {.fig.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule         {.fig.gz}{pdf}         {.fig.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule   {.CFree.fig}   {pdf}      {.CFree.fig.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule   {.CFree.fig.gz}{pdf}   {.CFree.fig.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule {.CMeFree.fig}   {pdf}    {.CMeFree.fig.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule {.CMeFree.fig.gz}{pdf} {.CMeFree.fig.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule{.CNonFree.fig}   {pdf}   {.CNonFree.fig.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule{.CNonFree.fig.gz}{pdf}{.CNonFree.fig.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}

% .m (matlab) -> .eps -> .pdf
\DeclareGraphicsRule  {.m}   {pdf}  {.m.tmp.pdf}{`bash -c 'file=$(basename #1);                            path=$(dirname #1); cd $path; if [ ! -f $file.tmp.pdf ] || [ $file.tmp.pdf -ot $file    ]; then       cat $file    > tmp.m; echo print -depsc tmp.eps >> tmp.m; cat tmp.m | matlab -nosplash; epstopdf tmp.eps -o $file.tmp.pdf; rm tmp.m tmp.eps; fi'}
\DeclareGraphicsRule  {.m.gz}{pdf}  {.m.tmp.pdf}{`bash -c 'file=$(basename #1); file=${file/.m.gz/.m};     path=$(dirname #1); cd $path; if [ ! -f $file.tmp.pdf ] || [ $file.tmp.pdf -ot $file.gz ]; then gunzip -c $file.gz > tmp.m; echo print -depsc tmp.eps >> tmp.m; cat tmp.m | matlab -nosplash; epstopdf tmp.eps -o $file.tmp.pdf; rm tmp.m tmp.eps; fi'}

% gp (gnuplot)
% png is better than jpg, however neither supports the linewidth option
% metapost is the best, you can use tex commands in titles etc
% I use pdf now, since metapost cannot be converted to bicolor or monocolor images for the CPL, if you want to return to metapost, simply replace pdf by mps in this section
\DeclareGraphicsRule         {.gp}   {pdf}            {.gp.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule         {.gp.gz}{pdf}         {.gp.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule   {.CFree.gp}   {mps}      {.CFree.gp.\CPL.tmp.mps}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.mps'}
\DeclareGraphicsRule   {.CFree.gp.gz}{mps}   {.CFree.gp.gz.\CPL.tmp.mps}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.mps'}
\DeclareGraphicsRule {.CMeFree.gp}   {pdf}    {.CMeFree.gp.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule {.CMeFree.gp.gz}{pdf} {.CMeFree.gp.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule{.CNonFree.gp}   {pdf}   {.CNonFree.gp.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule{.CNonFree.gp.gz}{pdf}{.CNonFree.gp.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
%\DeclareGraphicsRule {.gp}   {mps} {.gp.tmp.mps}{`bash -c '/home/wiskott/TEX/macros/myGraphicx-gp-mps #1'}
%\DeclareGraphicsRule {.gp.gz}{mps} {.gp.tmp.mps}{`bash -c 'file=$(basename #1); file=${file/.gp.gz/.gp}; path=$(dirname #1); cd $path; if [ ! -f $file.tmp.mps ] || [ $file.tmp.mps -ot $file.gz ]; then echo set terminal mp color > tmp.gp; gunzip -c $file.gz >> tmp.gp; gnuplot tmp.gp > $file.mp; rm tmp.gp; mpost $file.mp; rm $file.mp $file.mpx $file.log; mv $file.0 $file.tmp.mps; fi'}

% eps
\DeclareGraphicsRule         {.eps}   {pdf}            {.eps.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule         {.eps.gz}{pdf}         {.eps.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule   {.CFree.eps}   {pdf}      {.CFree.eps.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule   {.CFree.eps.gz}{pdf}   {.CFree.eps.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule {.CMeFree.eps}   {pdf}    {.CMeFree.eps.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule {.CMeFree.eps.gz}{pdf} {.CMeFree.eps.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule{.CNonFree.eps}   {pdf}   {.CNonFree.eps.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule{.CNonFree.eps.gz}{pdf}{.CNonFree.eps.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
%\DeclareGraphicsRule{.eps}   {pdf}{.eps.tmp.pdf}{`bash -c 'file=$(basename #1);                            path=$(dirname #1); cd $path; if [ ! -f $file.tmp.pdf ] || [ $file.tmp.pdf -ot $file    ]; then                      epstopdf $file -o=$file.tmp.pdf; fi'}
%\DeclareGraphicsRule{.eps.gz}{pdf}{.eps.tmp.pdf}{`bash -c 'file=$(basename #1); file=${file/.eps.gz/.eps}; path=$(dirname #1); cd $path; if [ ! -f $file.tmp.pdf ] || [ $file.tmp.pdf -ot $file.gz ]; then gunzip -c $file.gz | epstopdf -f >     $file.tmp.pdf; fi'}

% ps
\DeclareGraphicsRule         {.ps}   {pdf}            {.ps.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule         {.ps.gz}{pdf}         {.ps.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule   {.CFree.ps}   {pdf}      {.CFree.ps.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule   {.CFree.ps.gz}{pdf}   {.CFree.ps.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule {.CMeFree.ps}   {pdf}    {.CMeFree.ps.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule {.CMeFree.ps.gz}{pdf} {.CMeFree.ps.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule{.CNonFree.ps}   {pdf}   {.CNonFree.ps.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule{.CNonFree.ps.gz}{pdf}{.CNonFree.ps.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
%\DeclareGraphicsRule {.ps}   {pdf} {.ps.tmp.pdf}{`bash -c 'file=$(basename #1);                          path=$(dirname #1); cd $path; if [ ! -f $file.tmp.pdf ] || [ $file.tmp.pdf -ot $file    ]; then                      epstopdf $file -o=$file.tmp.pdf; fi'}
%\DeclareGraphicsRule {.ps.gz}{pdf} {.ps.tmp.pdf}{`bash -c 'file=$(basename #1); file=${file/.ps.gz/.ps}; path=$(dirname #1); cd $path; if [ ! -f $file.tmp.pdf ] || [ $file.tmp.pdf -ot $file.gz ]; then gunzip -c $file.gz | epstopdf -f >     $file.tmp.pdf; fi'}

% incremental buildup of figures
\DeclareGraphicsRule{*}{mps}{*}{}
\fi

% texfig
% export as Latex picture
% check http://www.xfig.org/userman/latex_and_xfig.html#PDFLaTeX for
% combined pdf/latex graphics, and http://docs.miktex.org/manual/texfeatures.html
% for hints on write18 and immediate
% make sure filename ends on TEX (TEX-CCBY seems to work as well) and use like
% \resizebox{\textwidth}{!}{\includeTexFig{\dir/../Figures/figureTEX}}
% mark equations in figure as special if using latex syntax
\providecommand{\includeTexFig}{}
\renewcommand{\includeTexFig}[1]{
\IfFileExists{#1.fig}{\def\TEXFigFilename{#1}}{}%
\IfFileExists{#1.CFree.fig}{\def\TEXFigFilename{#1.CFree}}{}%
\IfFileExists{#1.CMeFree.fig}{\def\TEXFigFilename{#1.CMeFree}}{}%
\IfFileExists{#1.CNonFree.fig}{\def\TEXFigFilename{#1.CNonFree}}{}%
\immediate\write18{file=$(basename \TEXFigFilename); path=$(dirname \TEXFigFilename); cd $path; if [ ! -f $file.fig.tmp.pdf ] || [ ! -f $file.fig.tmp.pdf_t ] || [ $file.fig.tmp.pdf_t -ot $file.fig ]; then fig2dev -L pdftex $file.fig $file.fig.tmp.pdf; fig2dev -L pdftex_t $file.fig $file.fig.tmp.pdf_t; fi}
\begin{picture}(0,0)%
\includegraphics{\TEXFigFilename.fig.tmp.pdf}%
\end{picture}%
\input{\TEXFigFilename.fig.tmp.pdf_t}
}
\DeclareGraphicsRule         {.fig.tmp.pdf}   {pdf}            {.fig.tmp.pdf.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule         {.fig.tmp.pdf.gz}{pdf}         {.fig.tmp.pdf.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule   {.CFree.fig.tmp.pdf}   {pdf}      {.CFree.fig.tmp.pdf.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule   {.CFree.fig.tmp.pdf.gz}{pdf}   {.CFree.fig.tmp.pdf.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule {.CMeFree.fig.tmp.pdf}   {pdf}    {.CMeFree.fig.tmp.pdf.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule {.CMeFree.fig.tmp.pdf.gz}{pdf} {.CMeFree.fig.tmp.pdf.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule{.CNonFree.fig.tmp.pdf}   {pdf}   {.CNonFree.fig.tmp.pdf.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}
\DeclareGraphicsRule{.CNonFree.fig.tmp.pdf.gz}{pdf}{.CNonFree.fig.tmp.pdf.gz.\CPL.tmp.pdf}{`bash -c 'make -f /home/wiskott/TEX/macros/myGraphicx-global.mk #1.\CPL.tmp.pdf'}

% for maximal size while maintaining the aspect ratio
%\includegraphics[keepaspectratio,totalheight=0.75\textheight,width=\textwidth]{...}

%\renewcommand{\includeTexFig}[1]{
%\immediate\write18{file=$(basename #1); path=$(dirname #1); cd $path; if [ ! -f $file.fig.tmp.pdf ] || [ ! -f $file.fig.tmp.pdf_t ] || [ $file.fig.tmp.pdf_t -ot $file.fig ]; then fig2dev -L pdftex $file.fig $file.fig.tmp.pdf; fig2dev -L pdftex_t $file.fig $file.fig.tmp.pdf_t; fi}
%\begin{picture}(0,0)%
%\includegraphics{#1.fig.tmp.pdf}%
%\end{picture}%
%\input{#1.fig.tmp.pdf_t}
%}


==> TEX-macros/myLatexOrPdflatex.tex <==
\providecommand{\latexOrPdflatex}[2]{\ifx\undefined\pdfoutput%
#1%
\else%
#2%
\fi}



==> TEX-macros/myLectureBody.tex <==
\input{./TEX-macros/myBasics}
\let\footnote=\endnote
\input{./TEX-macros/myLatexOrPdflatex}
\input{./TEX-macros/myMath}
\input{./TEX-macros/myUSEnglish}
\input{./TEX-macros/myFootnoteAddress}

%\input{myHyperref}
% see http://www.tug.org/applications/hyperref/manual.html#x1-90003.5
\usepackage[pagebackref=true,bookmarks=true,bookmarksopen=false,bookmarksnumbered=true,colorlinks=true]{hyperref}
%\hypersetup{a4paper,colorlinks=true,citecolor=blue,urlcolor=red,linkcolor=myGreen,% I have changed this line because of an error message from ShareLatex.
\hypersetup{colorlinks=true,citecolor=blue,urlcolor=red,linkcolor=myGreen,%
  pdftitle={},%
  pdfauthor={Laurenz Wiskott}}

\sloppy

\usepackage{natbib}
\bibliographystyle{apalike}
%\bibliographystyle{plainnat}

\usepackage{url}


\usepackage{wrapfig}

\usepackage{fp} % to provide fixed point arithmetic, see https://ctan.org/pkg/fp

%\input{myLatin}
\input{./TEX-macros/myUTF8}
\usepackage{float}

% A4 manuscript dimensions
\include{A4wide}
%\setlength{\parindent}{0em}
%\setlength{\parskip}{1.5ex plus 1.5ex minus0.5ex}

% caption definition of Rolf
\makeatletter
%
\long\def\@makecaption#1#2{%
   \vskip 10\p@
   \setbox\@tempboxa\hbox{{\bf #1: }#2}%
   \ifdim \wd\@tempboxa >\hsize
%       {\bf #1}#2\par  % original version
       {\bf #1: }#2\par
     \else
       \hbox to\hsize{\hfil\box\@tempboxa\hfil}%
   \fi}
%
\makeatother
%

% variable to decide whether to format the lecture notes for students or not
%\newboolean{StudentEdition}
%\setboolean{StudentEdition}{false}
% TODO: Replace this by a variable \Edition that assumes the values Me, Students, or Public.

\newboolean{LNSymbolsExplained}
\setboolean{LNSymbolsExplained}{false}
\newcommand{\EqnSymbol}{\blacklozenge}
\newcommand{\EqnLectSymbol}{\lozenge}
% \markText with underlines [does not work, this has trouble with citations]
%\usepackage{soul} \newcommand{\markTextCore}[1]{\ul{#1}} \newcommand{\martTextMark}{is underlined}\newcommand{\markByColor}[1]{#1}
% \markText with underlines
% \usepackage[normalem]{ulem} \newcommand{\markTextCore}[1]{\uline{#1}} \newcommand{\martTextMark}{is underlined}\newcommand{\markByColor}[1]{#1} % to provide underline with line breaks, see https://tex.stackexchange.com/questions/9550/why-does-underlined-text-not-get-wrapped-once-it-hits-the-end-of-a-line
% \markText with dark green
%\newcommand{\markTextCore}[1]{\textcolor{myDarkGreen}{#1}} \newcommand{\martTextMark}{is set in dark green}\newcommand{\markByColor}[1]{#1}
% \markText with dark red boldface
\newcommand{\markTextCore}[1]{\textcolor{myDarkRed}{\textbf{#1}}} \newcommand{\martTextMark}{is set in dark red boldface}\newcommand{\markByColor}[1]{{\color{myDarkRed}#1}}\newcommand{\markByColorSpace}{\hspace{0.6ex}}
% \markText with boldface
% \newcommand{\markTextCore}[1]{\textbf{#1}} \newcommand{\martTextMark}{(but not inline formulas) is set in bold face}\newcommand{\markByColor}[1]{#1}
\newcommand{\markText}[1]{\markTextCore{#1}}
\newcommand{\markEqn}{\EqnSymbol\phantom{|} \quad}
\newcommand{\markEqnLeft}{\EqnSymbol| \quad}
\newcommand{\markEqnLeftLect}{\EqnSymbol|\!\EqnLectSymbol \quad}
\newcommand{\markEqnLect}{\EqnLectSymbol\phantom{|} \quad}
\newcommand{\markEqnLectLeft}{\EqnLectSymbol| \quad}

%\newcommand{\LNhint}{$\to$}
\newcommand{\citeLN}[1]{\cite[$\to$][]{Wisk-LN-#1}}
%\newcommand{\LNTimeStamp}[1]{\ifthenelse{\boolean{StudentEdition}}{}{\marginpar{\mbox{--- #1 min ---}}}}
\newcommand{\LNTimeStamp}[1]{\ifthenelse{\equal{\LNEdition}{Me}}{\marginpar{\mbox{--- #1 min ---}}}{}}
%\newcommand{\LNTotalTimeStamp}{\ifthenelse{\boolean{StudentEdition}}{}{\marginpar{\mbox{--- \arabic{LNTotalTimeDesired} min ---}}}}
\newcommand{\LNTotalTimeStamp}{\ifthenelse{\equal{\LNEdition}{Me}}{\marginpar{\mbox{--- \arabic{LNTotalTimeDesired} min ---}}}{}}
\newcommand{\timeStamp}[1]{\LNTimeStamp{#1}}
%\newcommand{\LNTime}[1]{\ifthenelse{\boolean{StudentEdition}}{}{ (#1 min)}}
\newcommand{\LNTime}[1]{\ifthenelse{\equal{\LNEdition}{Me}}{ (#1 min)}{}}

\newcounter{LNTotalTimeDesired}

% \CPL is now defined in \myGraphix
\providecommand{\LNTimes}[2]{}
\providecommand{\LNTimess}[2]{}
\ifthenelse{\equal{\LNEdition}{Me}}{%
  \renewcommand{\LNTimes}[2]{ (#1/#2! min)}
  \renewcommand{\LNTimess}[2]{ (#1/#2! min --- \arabic{LNTotalTimeDesired} min)}
}{%
  \ifthenelse{\equal{\LNEdition}{Students}}{%
    \renewcommand{\LNTimes}[2]{}
    \renewcommand{\LNTimess}[2]{}
}{%
    \ifthenelse{\equal{\LNEdition}{Public}}{%
      \renewcommand{\LNTimes}[2]{}
      \renewcommand{\LNTimess}[2]{}
    }{%
      \LWUnknownCommandToStopLatexHereBecauseOfWrongEdition
    }}}
\input{./TEX-macros/myGraphicx}
%%% reference to slides
\providecommand{\RefToSlidesInHeader}{ ($\to$ slides)}

\input{./TEX-macros/myBeamerStyle} % Should come before the first use of CopyrightProtectionLevel but after the definition of \CPL and \markText etc.
\ifthenelse{\equal{\LNEdition}{Me}}{%
  \setcounter{CopyrightProtectionLevel}{1} % 0: no protection; 1: mark but show; 2: mark and hide
}{%
  \ifthenelse{\equal{\LNEdition}{Students}}{%
    \setcounter{CopyrightProtectionLevel}{0} % 0: no protection; 1: mark but show; 2: mark and hide
}{%
    \ifthenelse{\equal{\LNEdition}{Public}}{%
      \setcounter{CopyrightProtectionLevel}{2} % 0: no protection; 1: mark but show; 2: mark and hide
    }{%
      \LWUnknownCommandToStopLatexHereBecauseOfWrongEdition
    }}}

% A section I would usually skip, because it is too elementary.
\providecommand{\LNElementarySection}{$\box$}
% A section I would only bring if time permits.
\def\LNExtraSection{{\bf+}}
% A section I would usually skip, because it is too advanced.
\providecommand{\LNAdvancedSection}{$\star$}
%\providecommand{\LNExtra}{ $\star$}
\providecommand{\LNTODO}[1]{\ifthenelse{\equal{\LNEdition}{Me}}{\textbf{TODO: #1}}{}}
%\providecommand{\ENTODO}[1]{\ifthenelse{\boolean{StudentEdition}}{}{\textbf{TODO: #1}}}
\providecommand{\LNExtraInfo}[1]{\ifthenelse{\equal{\LNEdition}{Me}}{#1}{}}

\newcommand{\LNAlert}[1]{\ifthenelse{\equal{\LNEdition}{Me}}{

\vspace{1ex}

\noindent\fbox{\begin{minipage}{\textwidth}\begin{center}#1\end{center}\end{minipage}}

\vspace{1ex}

}{}}

% to add a continuation entry in the table of contents use
% \ifthenelse{\boolean{StudentEdition}}{}{
%  \section*                     {\quad\ Orthonormal basis systems (cont.)\LNTimes{90}{90}}
%  \addcontentsline{toc}{section}{\quad\ Orthonormal basis systems (cont.)\LNTimes{90}{90}}
% }

%%% beamer compatibility macros

\renewcommand{\SectionHeader}[2][]{}
%\renewcommand{\SlideHeader}[1]{}
%\setlength{\freeheight}{0.4\textheight}
%\renewcommand{\Source}[1]{}
%\renewcommand{\note}[1]{#1}

% TODO: Understand how the definition of an environment with optional
 % parameters works and redefine 'frame' such that
 % /home/wiskott/PR/General/Talks/Slides/Summary.tex works
%\renewenvironment{frame}[1]{I want this to be seen this is the beginning #1}{this is the end}

\renewcommand{\frame}[1]{}
%\renewcommand{\note}[1]{\noindent\begin{minipage}[c]{0.48\textwidth} #1 \end{minipage}}
\providecommand{\note}{}
\renewcommand{\note}[1]{#1}

% define lengths for \inputSlide
\newlength{\LNSlideWidth}  \setlength{\LNSlideWidth}{0.7\textwidth}
\newlength{\LNSlideHeight} \setlength{\LNSlideHeight}{0.84\LNSlideWidth}
\newlength{\LNWrapWidth}   \setlength{\LNWrapWidth}{\LNSlideWidth}

\providecommand{\inputSlide}{}
\renewcommand{\inputSlide}[1]{

\vspace*{\fill}

\noindent
\begin{minipage}[t]{\textwidth}
\begin{wrapfigure}{l}{\LNWrapWidth}

\vspace{-2.3ex}

\fbox{\begin{minipage}[b][\LNSlideHeight][t]{\LNSlideWidth}\hspace*{-0.5ex}\centerline{\includeslide[width=1.16\textwidth]{slide:\dir/#1}}\end{minipage}}
\vspace{-3ex} % determines distance between bottom line of image and top line of regular text under the image
\end{wrapfigure}

 \quad \vspace{-2ex}

 \input{\dir/#1}

 \vspace{1ex}

\end{minipage}%
\rule[-\LNSlideHeight]{0ex}{\LNSlideHeight}

\vspace*{\fill}

\pagebreak[3]

}

\providecommand{\inputSlideC}{}
\renewcommand{\inputSlideC}[1]{

\vspace*{\fill}

\noindent
\begin{minipage}[t]{\textwidth}
\begin{wrapfigure}{l}{\LNWrapWidth}

\vspace{-2.3ex}

\ifthenelse{\value{CopyrightProtectionLevel}<1}{\fbox{\begin{minipage}[b][\LNSlideHeight][t]{\LNSlideWidth}\hspace*{-0.5ex}\centerline{\includeslide[width=1.16\textwidth]{slide:\dir/#1}}\end{minipage}}}{}
\ifthenelse{\value{CopyrightProtectionLevel}=1}{\fbox{\begin{minipage}[b][\LNSlideHeight][t]{\LNSlideWidth}\hspace*{-0.5ex}\centerline{\includeslide[width=1.16\textwidth]{slide:\dir/#1}\llap{\includegraphics[width=1\textwidth]{/home/wiskott/PR/General/Talks/Figures/ProtectCopyrights}}}\end{minipage}}}{}
\ifthenelse{\value{CopyrightProtectionLevel}>1}{\fbox{\begin{minipage}[b][\LNSlideHeight][t]{\LNSlideWidth}\hspace*{-0.5ex}\centerline{\includegraphics[width=1\textwidth]{/home/wiskott/PR/General/Talks/Figures/ProtectCopyrights}}\end{minipage}}}{}
\vspace{-3ex} % determines distance between bottom line of image and top line of text under the image
\end{wrapfigure}

 \quad \vspace{-2ex}

 \input{\dir/#1}

 \vspace{1ex}

\end{minipage}%
\rule[-\LNSlideHeight]{0ex}{\LNSlideHeight}

\vspace*{\fill}

\pagebreak[3]

}
\renewcommand{\inputSlideC}[1]{\inputSlide{#1}}

\newcommand{\LNExtraQuestion}[1]{
  \ifthenelse{\equal{\LNEdition}{Me}}{
    \textbf{Extra question:}#1
  }{}
}

%==============================================================================

\ignore{
\providecommand{\inputSlide}{}
\renewcommand{\inputSlide}[1]{
\noindent
\fbox{%
\begin{minipage}{0.48\textwidth}
%\includeslide[width=\textwidth]{slide:\SlidesSection:#1} 
\includeslide[width=\textwidth]{slide:\dir/#1} 
\end{minipage}%
}\hfill
\begin{minipage}{0.48\textwidth} 
\input{\dir/#1}
\quad 
\end{minipage}

}
}%\ignore{

\ignore{
\usepackage{wrapfig}
\renewcommand{\inputSlide}[1]{

\vspace*{\fill}

\noindent
\begin{minipage}[t]{\textwidth}
\begin{wrapfigure}[16]{l}{0.5\textwidth}

\vspace{-2.3ex}

%\fbox{\includeslide[width=0.487\textwidth]{slide:\SlidesSection:#1}}
\fbox{\includeslide[width=0.487\textwidth]{slide:\dir/#1}}

%\vspace{-1ex}

\end{wrapfigure}

 \quad \vspace{-2ex}

 \input{\dir/#1}

 \vspace{1ex}

\end{minipage}%
%\rule[-0.24\textheight]{0ex}{0.24\textheight}
\rule[-0.23\textheight]{0ex}{0.23\textheight}

\vspace*{\fill}

\pagebreak[3]

}
}%\ignore{


==> TEX-macros/myLectureNotes.tex <==
\usepackage{endnotes}

\usepackage[noamsthm]{beamerarticle}
\input{./TEX-macros/myLectureBody}

\usepackage{pgf}

\def\LNMaketitle#1#2#3{
  \LNMaketitleAuthors{#1}{#2}{Laurenz Wiskott \\ Institut f\"ur Neuroinformatik \\ Ruhr-Universit\"at Bochum, Germany, EU}{#3}
}

\def\LNMaketitleAuthors#1#2#3#4{
  
  \title{\footnotetext{\copyright{} #2{} Laurenz Wiskott (ORCID
      \url{http://orcid.org/0000-0001-6237-740X}, homepage
      \url{https://www.ini.rub.de/PEOPLE/wiskott/}). \ifthenelse{\value{CopyrightProtectionLevel}<2}{Do
        not distribute these lecture notes!  This version is only for the personal use of
        my students.}{This work (except for all figures from other sources, if present)
        is licensed under the Creative Commons Attribution-ShareAlike 4.0 International
        License, see \url{http://creativecommons.org/licenses/by-sa/4.0/}.  If figures
        are not included for copyright reasons, they are uni colored, but the word
        'Figure', 'Image', or the like in the reference is often linked to a freely
        available copy.}
      \\
      % \ifthenelse{\boolean{LNSymbolsExplained}}{}{\footnotemark\footnotetext{
      \EG{Core text and formulas are set in dark red, one can repeat the lecture notes
        quickly by just reading these; $\EqnSymbol$~marks important formulas or items
        worth remembering and learning for an exam; $\EqnLectSymbol$~marks less important
        formulas or items that I would usually also present in a lecture;
        \LNExtraSection~marks sections that I would usually skip in a lecture.}{Wichtige
        Textstellen (nicht aber Formeln im Fließtext) sind fett gedruckt;
        $\EqnSymbol$~markiert wichtige abgesetzte Formeln oder Strichpunkte, die man sich
        merken sollte; $\EqnLectSymbol$~markiert weniger wichtige abgesetzte Formeln oder
        Strichpunkte, die ich in der Vorlesung aber auch diskutiere;
        \LNExtraSection~markiert Abschnitte, die ich in der Regel nicht in der Vorlesung
        behandle.}
      % }}\setboolean{LNSymbolsExplained}{true}
  \\
  More teaching material is available at
  \url{https://www.ini.rub.de/PEOPLE/wiskott/Teaching/Material/}.  } \textbf{#1 \\ {\large --- Lecture Notes ---} } }
  
 \author{#3}

 \date{#4}

\maketitle

}

%\def\LNAppearance#1{\ifthenelse{\boolean{StudentEdition}}{}{#1}}
\def\LNAppearance#1{\ifthenelse{\equal{\LNEdition}{Me}}{#1}{}}

\def\LNLecture#1#2#3{
  \pagebreak[3]
  \vspace{4ex}
  % \addcontentsline{toc}{section}{LECTURE #1/#2 #3}
  % - obsolete, it adds minutes, e.g. 1/2 (88/90! min), but I don't use that anymore
  \ifthenelse{\equal{\LNEdition}{Me}}{%
    \addcontentsline{toc}{section}{LECTURE #1/#2}
  }{%
    \ifthenelse{\equal{\LNEdition}{Students}}{%
      \addcontentsline{toc}{section}{LECTURE #1/#2}
    }{%
      \ifthenelse{\equal{\LNEdition}{Public}}{%
      }{%
        \LWUnknownCommandToStopLatexHereBecauseOfWrongEdition
      }}}
  \begin{minipage}{\textwidth}
    % \section*{LECTURE #1/#2 #3}
    \ifthenelse{\equal{\LNEdition}{Me}}{%
      \rule{\textwidth}{1ex}
      \section*{LECTURE #1/#2}
      \rule{\textwidth}{1ex}
    }{%
      \ifthenelse{\equal{\LNEdition}{Students}}{%
        \section*{LECTURE #1/#2}
      }{%
        \ifthenelse{\equal{\LNEdition}{Public}}{%
        }{%
          \LWUnknownCommandToStopLatexHereBecauseOfWrongEdition
        }}}
  \end{minipage}
  \nopagebreak
}

% 2018-08-08 I have introduced the 'Unit' version for the PCA lecture notes.
% It allows me to distinguish between regular lectures and flipped classroom (units).
% But for the time being I use the term 'lecture' throughout.
\def\LNUnit#1#2#3{
%\ifthenelse{\boolean{StudentEdition}}{}{%
\vspace{2ex}
\pagebreak[3]
%\addcontentsline{toc}{section}{LECTURE #1/#2 #3}
\addcontentsline{toc}{section}{LECTURE #1/#2}
\begin{minipage}{\textwidth}
\rule{\textwidth}{1ex}
%\section*{LECTURE #1/#2 #3}
\section*{LECTURE #1/#2}
\rule{\textwidth}{1ex}
\end{minipage}
%}%\ifthenelse{\boolean{StudentEdition}}{}{%
}



==> TEX-macros/myMath.tex <==
% see http://www.ams.org/tex/amslatex.html
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{xfrac}% http://ctan.org/pkg/xfrac
\usepackage{bm}

\def \stackref #1#2{\stackrel{\mbox{\tiny (#1)}}{#2}}
\def \stackphantom #1#2{\stackrel{\phantom{\mbox{\tiny (#1)}}}{#2}}
%\def \vec #1{{\bf{}#1}} % does not make greek letters boldface
%\def \vec #1{{\boldsymbol{}#1}} % does not work
%\def \vec #1{\boldmath{#1}} % does not make greek letters boldface
%\def \vec #1{\mathbf{#1}} % does not make greek letters boldface
%\def \vec #1{\bm{#1}} % does not work in headers, plots symbols straight not italic
\def \vec #1{\texorpdfstring{\bm{#1}}{#1}}
\def \mat #1{\texorpdfstring{\bm{#1}}{#1}}

% See https://tex.stackexchange.com/questions/174840/bmp-in-the-section-title-or-subsection-title-produces-error
% does not compile
%\DeclareRobustCommand{\vec}[1]{\bm{#1}}
%\pdfstringdefDisableCommands{%
%  \renewcommand{\vec}[1]{#1}%
%}
%\DeclareRobustCommand{\mat}[1]{\bm{#1}}
%\pdfstringdefDisableCommands{%
%  \renewcommand{\mat}[1]{#1}%
%}

\def \dd {\text{d}}
\def \ee {\text{e}}
\def \ii {\text{i}}
\def \argmin {\text{arg min}}
\def \grad {\text{grad}}
\def \trace {\text{tr}}
\def \sgn {\text{sgn}}

% use \mathbb{..} for number sets

==> TEX-macros/myRootDir.tex <==
\def\RootDir{/home/wiskott}


==> TEX-macros/myRotating.tex <==
\usepackage{rotating}

==> TEX-macros/myUSEnglish.tex <==
%\usepackage[latin1]{inputenc}       % allow Latin1 characters % I use utf8 now
%\usepackage[greek,german,USenglish]{babel} % (greek for the euro sign)
%\def \Euro{\textgreek{\euro}}
\usepackage[german,USenglish]{babel} % (the euro sign is now provided in myUTF8)

\providecommand \EG[2]{}
\renewcommand \EG[2]{#1}
\providecommand \E[1]{}
\renewcommand \E[1]{#1}
\providecommand \G[1]{}
\renewcommand \G[1]{}

\providecommand{\Eword}[1]{}
\renewcommand{\Eword}[1]{ \textnormal{(E: #1)}}
\providecommand{\EWord}[1]{}
\renewcommand{\EWord}[1]{\Eword{#1}}

\providecommand{\Gword}[1]{}
\renewcommand{\Gword}[1]{ \textnormal{(D: #1)}}
\providecommand{\GWord}[1]{}
\renewcommand{\GWord}[1]{\Gword{#1}}



==> TEX-macros/myUTF8.tex <==
\usepackage[utf8]{inputenc}
\usepackage{eurosym}
\DeclareUnicodeCharacter{20AC}{\euro} % This should allow me to use € directly in the source text, see http://www.theiling.de/eurosym.html
\usepackage{textcomp}
\DeclareUnicodeCharacter{C2B0}{\textdegree} % This should allow me to use ° directly in the source text, see http://en.wikibooks.org/wiki/LaTeX/Special_Characters#Degree_symbol_for_temperature_and_math
% See http://www.utf8-zeichentabelle.de/ for more utf8 unicode codes
% http://www.sql-und-xml.de/unicode-database/
% http://www.fileformat.info/info/unicode/

